Gibbs measures have local product structure

It is well-known that equilibrium measures for uniformly hyperbolic dynamical systems have a local product structure, which plays an important role in their mixing properties. Existing proofs of this fact rely either on transfer operators or on leafwise constructions, and in particular are not well-suited to the approach to thermodynamic formalism based on Bowen's specification property. Here we provide an alternate proof based on the Gibbs property, which fits more comfortably in that approach.

==> mymacros.tex <==
\newcommand{\foot}[1]{\mbox{}\marginpar{\raggedleft\hspace{0pt}\tiny #1}}
%\newcommand{\foot}[1]{}
%\newcommand{\vc}[1]{\foot{VC: #1}}
\newcommand{\fixnow}[1]{\foot{\color{red} #1}}

\newcommand{\deleted}[1]
{}
%{\sout{#1}}
\newcommand{\modified}
{}
%{\color{blue}}

\newcommand{\msout}[1]{\text{\deleted{\ensuremath#1}}}


\newcommand{\ph}{\varphi}
\newcommand{\eps}{\epsilon}
\newcommand{\ulim}{\varlimsup}
\newcommand{\llim}{\varliminf}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\AAA}{\mathcal{A}}
\newcommand{\BBB}{\mathcal{B}}
\newcommand{\OOO}{\mathcal{O}}
\newcommand{\CCC}{\mathcal{C}}
\newcommand{\DDD}{\mathcal{D}}
\newcommand{\III}{\mathcal{I}}
\newcommand{\LLL}{\mathcal{L}}
\newcommand{\FFF}{\mathcal{F}}
\newcommand{\EEE}{\mathcal{E}}
\newcommand{\MMM}{\mathcal{M}}
\newcommand{\SSS}{\mathcal{S}}
\newcommand{\UUU}{\mathcal{U}}
\newcommand{\MF}{\mathcal{M}_F}
\newcommand{\MFe}{\mathcal{M}_F^e}
\newcommand{\RRR}{\mathcal{R}}
\newcommand{\PPP}{\mathcal{P}}
\newcommand{\GGG}{\mathcal{G}}
\newcommand{\QQQ}{\mathcal{Q}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\dS}{d_\mathrm{S}}
\newcommand{\dK}{d_\mathrm{K}}
\newcommand{\di}{\partial}
\newcommand{\ideal}{\di\tilde M}
\newcommand{\Vl}{V_{\mathrm{loc}}}
\renewcommand{\L}{{\Lambda}}
\newcommand{\htop}{h_{\mathrm{top}}}
\newcommand{\one}{\mathbf{1}}
\DeclareMathOperator{\Leb}{Leb}
\DeclareMathOperator{\Comp}{Comp}
\DeclareMathOperator{\diam}{diam}
\newcommand{\Zspan}{Z^\mathrm{span}}
\newcommand{\Zsep}{Z^\mathrm{sep}}
\newcommand{\Es}{E^\mathrm{s}}
\newcommand{\Eu}{E^\mathrm{u}}
\newcommand{\Ws}{W^\mathrm{s}}
\newcommand{\Wu}{W^\mathrm{u}}
\newcommand{\Wsl}{\Ws_\mathrm{loc}}
\newcommand{\Wul}{\Wu_\mathrm{loc}}
\newcommand{\Wcs}{W^\mathrm{cs}}
\newcommand{\Wcu}{W^\mathrm{cu}}
\newcommand{\Ps}{P^\mathrm{s}}
\newcommand{\Pu}{P^\mathrm{u}}
\newcommand{\ms}{m^\mathrm{s}}
\newcommand{\mmu}{m^\mathrm{u}}
\newcommand{\mf}{m^+}
\newcommand{\mb}{m^-}
\newcommand{\bm}{\lambda}
\newcommand{\cm}{\nu}
\newcommand{\Gam}{\Gamma}
\newcommand{\hgood}{\hat{h}}
\newcommand{\hbad}{h^*}
\newcommand{\xminus}{x.}
\newcommand{\yminus}{y.}
\newcommand{\zminus}{z.}
\newcommand{\xplus}{.x}
\newcommand{\du}{\rho^u}
\newcommand{\ds}{\rho^s}
\newcommand{\Lambdap}{\Lambda^+}
\newcommand{\lLambdap}{\underline{\Lambda}^+}
\newcommand{\uLambdap}{\bar{\Lambda}^+}
\newcommand{\uQ}{\overline{Q}}
\newcommand{\lQ}{\underline{Q}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{thma}{Theorem}
\newtheorem*{thma*}{Theorem}
\renewcommand{\thethma}{\Alph{thma}}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem*{problem}{Problem}
\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{construction}[theorem]{Construction}


